Survey of Learning-based Approaches for Robotic In-Hand Manipulation

Human dexterity is an invaluable capability for precise manipulation of objects in complex tasks. The capability of robots to similarly grasp and perform in-hand manipulation of objects is critical for their use in the ever changing human environment, and for their ability to replace manpower. In recent decades, significant effort has been put in order to enable in-hand manipulation capabilities to robotic systems. Initial robotic manipulators followed carefully programmed paths, while later attempts provided a solution based on analytical modeling of motion and contact. However, these have failed to provide practical solutions due to inability to cope with complex environments and uncertainties. Therefore, the effort has shifted to learning-based approaches where data is collected from the real world or through a simulation, during repeated attempts to complete various tasks. The vast majority of learning approaches focused on learning data-based models that describe the system to some extent or Reinforcement Learning (RL). RL, in particular, has seen growing interest due to the remarkable ability to generate solutions to problems with minimal human guidance. In this survey paper, we track the developments of learning approaches for in-hand manipulations and, explore the challenges and opportunities. This survey is designed both as an introduction for novices in the field with a glossary of terms as well as a guide of novel advances for advanced practitioners.

==> IL.tex <==
% Focus, polish, divide to subsections

As discussed in the previous section, training RL policies for real robots from scratch is usually time-consuming and often infeasible due to the lack of sufficient data \citep{rapisarda2019reinforcement}. A prominent approach for coping with these challenges is Imitation Learning (IL). Instead of learning a skill without prior knowledge, IL aims to learn from expert demonstrations \citep{Duan2017,fang2019survey}. Prior knowledge from the expert can then be optimized for the agent through some learning framework such as RL. While IL is often considered a sub-field of RL, we provide a distinct focus due to its importance and wide work. IL can be categorized into two main approaches: Behavioral Cloning (BC) and Inverse Reinforcement Learning (IRL) % and Generative Adversarial Imitation Learning (GAIL) 
\citep{zheng2022imitation}. In BC, a policy is trained in a supervised learning fashion with expert data to map states to actions. IRL, on the other hand, extracts the reward function from the expert data in order to train an agent with the same preferences \citep{Arora2021}. 

In both BC and IRL, a policy is learned with some prior. This is in contrast to RL where the policy is learned from scratch based on the agent's own experience. Hence, IL requires an initial process of data acquisition as illustrated in Figure \ref{fig:IL_FC}. First, data is collected from demonstrations of an expert. Demonstrations can be acquired in various mediums such as recording human motion or recording proprioceptive sensing of the robot during manual jogging. In the next step, IL usually involves either learning a policy to directly imitate the demonstration (BC) or feature extraction from the data (IRL). The last step is further policy refinement through conventional RL. From an RL perspective, IL usually reduces the learning time by bootstrapping the learning process using an approximation of the expert's policy. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[]
\centering
% 	\includegraphics
	% [scale=0.4]{figures/ILFlow.jpg}
\begin{mybox}{Data Acquisition}{\faIcon[regular]{camera}}{gray!80!red}{4cm}
\begin{itemize}
    \item Teleoperation \citep{Arunachalam2023,Kumar2016b}
    \item Object-centric \citep{Gupta2016}
    \item Video of human or robot \citep{Arunachalam2023, Arunachalam2023holo}
    \item Manual motion of the robot \citep{Li2014,Gaspar2018}
    % \item EMG recordings
\end{itemize}
% 3-D model of hand using 3-D camera, 
\end{mybox}
\begin{mybox}{Learning Process}{\faIcon[regular]{university}}{gray!80!green}{3.4cm}
\begin{itemize}
    \item Behavioral Cloning (BC)
    \item Inverse Reinforcement Learning (IRL)
    \item Generative Adversarial Imitation Learning (GAIL) \citep{Wei2023}
\end{itemize}
%, Generative Adversarial Imitation Learning (GAIL)
\end{mybox}
\begin{mybox}{Policy Refinement}{\faIcon[regular]{trophy}}{green!60!gray}{2.2cm}
\begin{itemize}
    \item Reinforcement learning
\end{itemize}
\end{mybox}
\vspace{-0.02in}
\caption{Flowchart of policy training with Imitation Learning (IL).}%\citep{hussein2017imitation}}
\label{fig:IL_FC}
\end{figure} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ------------------------------------------

\subsection{Date Acquisition}

Data is collected from an expert demonstrator while conducting the desired task. The motion of the expert is recorded through some set of sensors such that the learning agent can later observe and learn to imitate. There are various approaches to demonstrate and record the motions and their choice may affect the learning process. 

One data acquisition approach is to teleoperate the robot throughout the task using designated tools such as a remote control \citep{zhang2018deep}. However, remote controls are unnatural and quite infeasible in teleoperation of dexterous robotic hands. In a more natural approach, \cite{Arunachalam2023} used a visual hand pose estimation model (i.e., skeleton) to approximate keypoints on the human hand during reorientation of an object. The user can also use a VR set in order to have the point-of-view of the robot \citep{Arunachalam2023holo}. In these examples, a policy is learned for an anthropomorphic robot hand by using simpler nearest-neighbors search in the data. The action in the demonstration data which has a state closest to the current state is exerted. Similarly, \cite{Kumar2016b} recorded the proprioceptive state of a virtual anthropomorphic robotic hand during teleoperation with the CyberGlove worn by an expert user. With the glove, the joint angles along with tactile information are recorded. The recorded tasks are then used to train and evaluate in-hand manipulation with a five-finger dexterous hand for reorientation tasks. In a similar approach, \cite{wei2023wearable} designed a wearable robotic hand for IL teleoperation such that the expert has tactile feedback during demonstrations.

In a different approach by \cite{Gupta2016}, only information regarding the motion of a manipulated object is collected while ignoring the motions of the human expert. Hence, an object-centric policy is learned while selecting the most relevant demonstration for each initial state in the training. In a different approach, the demonstrator manually moves the robot by contacting and pushing it to perform the task \citep{Li2014,Shin2024,Gaspar2018}. During the demonstration, the robot collects kinesthetic data from the joints. While the approach is simple, it is usually applied to robotic arms with a single serial kinematic chain. It is quite infeasible for a human to synchronously move a dexterous and multi-contact robotic hand to perform a complex in-hand manipulation task. Nevertheless, simpler tasks with non-dexterous hands may by possible while the authors have not found prior work.


% Some works collect images from the point of view of the robot during the manipulation of objects during VR-based teleoperation of the robot by an expert user \citep{zhang2018deep,Arunachalam2023holo,Arunachalam2023}.
%propose a VR teleoperation system that collects high-quality robotic manipulation demonstrations for visuomotor learning. 
% With the data, policies based on CNN, such as GoogLeNet and ImageNet, were trained and evaluated. Hence, the proposed method transforms pixel values in the images into actions using only a small amount of training data. %Only some of the demonstrated tasks involve in-hand manipulation, such as grasping cloth, which requires some pre-grasping manipulation.

 %Other approaches for collecting demonstration data include a joystick \citep{Zhu2018}, 

%Therefore, % to track by using RL in order to optimize a collection of controllers. It extends the guided policy search framework in order to find new initial conditions by generalizing NN policies. In addition, the authors use GPS in order to train the nonlinear NN policies that combine the capabilities of all of the controllers.

% Kumar et al. \citep{Kumar2016b} present learning-based approaches for feedback control of a dexterous five-finger hand performing non-prehensile manipulation. The authors show two main cases: predefined initial state and generalizing initial conditions. For generalizing initial conditions, they compare two approaches: deep learning, and nearest neighbors. The conclusion is that there are advantages and drawbacks to each approach and it seems that a combination between them will yield the best solution. In addition, the authors show local trajectory-based controllers for complex non-prehensile manipulation tasks can be constructed from small amounts of training data, and collections of such controllers can be interpolated to form more global controllers.

% Demonstration data collection can be done via tactile sensory gloves like the CyberGlove \citep{Funabashi2015}. %add examples. 
% This method allows the neural network to be built to accept tactile sensory, and use human demonstrations for the beginning of the training process. The authors collect a comprehensive dataset of manipulation tasks on a few specific objects, and successfully transfer the training to be used on new, previously untrained objects. 
 %present a robust method for generating in-hand manipulation for object and shapes that it had not been trained with. The authors develop deep NN that needs less training examples in comparison to feed-forward interpolation control. The deep NN is based upon predicting the next step joint angle based on current joint angle and touch state as well as physical parameters such as object size and shape.\\

% ------------------------------------------

\subsection{Learning Process}

% Training a policy based only on demonstrations
The process for learning from the demonstrations is commonly conducted by either BC or IRL \citep{hussein2017imitation}. In BC, the agent is required to directly take the strategy of the expert observed in the demonstrations \citep{Arunachalam2023}. The agent will exert an action taken by the expert when in a similar state. Hence, demonstration data is usually recorded in the form of state-action pairs which is easy to learn. Then, a policy is learned in a supervised learning manner. However, state-action pairs can be difficult to obtain from, for instance, video data. To cope with this problem, \cite{radosavovic2020state} proposed the state-only imitation learning (SOIL) approach where an inverse dynamics model can be trained to extract the actions chosen based on the change in the state perceived from videos. The inverse dynamics model and the policy are trained jointly. SOIL enables learning from demonstrations originating from different but related settings. While not an IL approach, \cite{Yuan2023} considered a trained teacher policy as an expert and used BC to distill it to a student in the training of in-hand manipulation with vision and tactile sensing. In a different work, BC was used to control a unique design of a gripper having actuated rollers on its fingertips \citep{Yuan2020}. The demonstration data was extracted from a handcrafted controller and shown to improve performance.

\cite{Rajeswaran2017} compared methods of RL to solve complex manipulation tasks, with and without incorporating human demonstrations. The authors suggested a method of incorporating demonstrations into policy gradient methods for manipulation tasks. The proposed Demonstration Augmented Policy Gradient (DAPG) method uses pre-training with BC to initialize the policy and an augmented loss function to reduce ongoing bias toward the demonstration. The results in the paper showcase that DAPG policies can acquire more human-like motion compared to RL from scratch and are substantially more robust. In addition, the learning process is considerably more sample-efficient. \cite{Jain2019} extended the work by exploring the contribution of demonstration data to visuomotor policies while being agnostic about the data's origin. Demonstrations were shown to improve the learning rate of these policies in which they can be trained efficiently with a few hundred expert demonstration trajectories. In addition, tactile sensing was found to enable faster convergence and better asymptotic performance for tasks with a high degree of occlusions. While \citeauthor{Rajeswaran2017} and \citeauthor{Jain2019} demonstrated the approach only in simulations, \cite{zhu2019dexterous} demonstrated the use of DAPG on a real-robot in complex dexterous manipulation tasks. The results have shown a decrease of training time from 4-7 hours to 2-3 hours by incorporating human demonstrations. 

Few studies on in-hand manipulation have used BC due to the significant effort required to collect sufficient demonstration data. While simple to implement, BC usually requires large amounts of data for sufficient performance \citep{Ross2011}. IRL, on the other hand, directly learns the reward function of the demonstrated expert policy which prioritizes some actions over others \citep{Arora2021}. IRL learns the underlying reward function of the expert which is the best definition of a task. Once acquired the reward function, an optimal policy can be trained to maximize such a reward using a standard RL algorithm. While general work on IRL is wide for various robotic applications, not much work has been done that combines IRL with in-hand manipulation. A single work demonstrated the IRL approximation of the reward function using expert samples of desired behaviours \citep{Orbik2021}. However, the authors have argued that the learned reward functions are biased towards the demonstrated actions and fail to generalize. Randomization and normalization were used to minimize the bias and enable generalization between different tasks. 

While not directly IRL, \cite{deng2020learning} utilized reward-shaping to improve the RL training of in-hand manipulation with a dexterous hand. By observing hand synergies of a human demonstrator, a limited and low-dimensional state space was constructed. Using reward-shaping allows the inclusion of multiple levels of knowledge, from the standard extrinsic reward to hand synergies-based reward and an uncertainty-based reward function that is aimed at directing efficient exploration of the state space. Learning using all three reward functions is shown through simulations to improve learning. The minor use of IRL to address in-hand manipulation problems may be explained by its tendency to provide ill-behaved reward functions and unstable policies \citep{cai2019global}.

IL was also proposed for in-hand manipulation without the use of RL. \cite{Solak2019} proposed the use of Dynamical Movement Primitives (DMP) \citep{Ijspeert2013}. The approach shows that a multi-finger dexterous hand can perform a task based on a single human demonstration while being robust to changes in the initial or final state, and is object-agnostic. However, the former property may yield object slip and compromise grasp stability. Hence, an extended work proposed haptic exploration of the object such that the manipulation is informed by surface normals and friction at the contacts \citep{Solak2023}. 


% GAIL
While traditional IRL has shown high performance in a wide range of tasks, it only provides a reward function that implicitly explains the experts' behaviour but does not provide the policy dictating what actions to take. Hence, the agent will still have to learn a policy through RL training in a rather expensive process. To address this problem, the Generative Adversarial Imitation Learning (GAIL) \citep{Ho2016} was proposed and combines IL with Generative Adversarial Networks (GAN) \citep{Goodfellow2020}. Similar to GAN, GAIL incorporates a generator and a discriminator. While the generator attempts to generate a policy that matches the demonstrations, the discriminator attempts to distinguish between data from the generator and the original demonstration data. Training of GAIL is, therefore, the minimization of the difference between the two. Consequently, GAIL is able to extract a policy from the demonstration data. Recently, the use of GAIL was proposed for in-hand manipulation by a dexterous hand \citep{Wei2023}. The approach was shown to perform significantly better than BC or direct RL training. GAIL has the potential to improve and expedite policy learning of more complex in-hand manipulation tasks, and should be further explored.

%Demonstration data was collected with a glove and a policy was trained for a simulated hand. Then, the policy was transferred to a real hand through visual perception.

% ------------------------------------------

% \subsection{Integrating demonstrations to RL}

% IL is used many times to pre-train or bootstrap a policy prior to applying an RL training process \citep{pfeiffer2018reinforced,ramirez2022model}. In such a way, the policy requires much less episodic interaction with the environment to perform well.

%In addition of using RL for refining imitation policies, IL can be used to bootstrap RL policies.





% Demonstrations have been shown to improve the learning rate for deep visuomotor policies for a variety of manipulation tasks with a simulated five-fingered dexterous hand \citep{Jain2019}. These policies directly control the hand using high-dimensional visual observations of the world and proprioceptive observations from the robot and can be trained efficiently with a few hundred expert demonstration trajectories. They also find that using touch-sensing information enables faster learning and better asymptotic performance for tasks with a high degree of occlusions. The core algorithm is based upon a CNN for deducing the robot hand action and policy. The offered architecture is done as IL since RL was found to be inefficient. The IL is trained with a few hundred expert demonstrations in under one hour on a single workstation.



% Zhu et al. \citep{zhu2019dexterous} developed an end-to-end approach for direct mapping of the sensor reading to action, without the need for task-specific models or policy classes. The learning process is done entirely in reality, without the aid of simulations, and while learning skills took 4-7 hours using pure RL, adding a small number of simulations using DAPG shortened the learning time to 2-3 hours.  

% Avishai: There is no in-hand manipulaiton here
% Meta-learning processes, where policies are trained on diverse tasks, in robotic manipulation involving a variety of objects or environments, aim to improve the ability to generalize to related tasks \citep{xu2018meta}. A common goal for meta-learning is for the learner to generalize with minimal training attempts on the new scenario, termed few-shot, one-shot, or ideally, zero-shot learning. \citep{Zhu2018a} combine reinforcement and imitation learning into one. In their paper they show that their approach considerably improves significantly the ability to train systems that combines challenging dexterous manipulation tasks from visual systems. According to their experiments, the combined method has better performances in comparison to agents trained with RL or IL alone. In addition, the authors illustrate that the achieved policies, trained with large visual and dynamics variations, can achieve preliminary successes in zero-shot sim2real transfer. Their offered method is implemented in a three-stage pipeline. In the first stage, the exploration problem is simplified by collecting a small amount of demonstration data. In the second stage, the method uses a physical simulation to perform large-scale robot training. In the final stage, sim2real  transfer is performed for real-world deployment. % different Zhu from previous citation, how to differentiate? This is in arxiv only, but highly cited, consider keeping/removing. Haven't polished the paragraph yet in case we remove the citation.

% Impedance control, used successfully in model-based RL schemes, can be improved with demonstrations as well. Li et al. \citep{Li2014} offer a new method for learning the object’s manipulation impedance (stiffness) using data obtained from human demonstration. The approach decomposes the object’s impedance into two complementary components, the impedance for stable grasping and the impedance for object manipulation. For dexterous manipulation, the desired reference trajectory and the desired object impedance are learned through an optimization-based approach. Both of these approaches are validated on a multi-fingered robotic hand. The results show that learning from human demonstration is an effective way to specify the desired impedance for object-centric tasks. Caldas et al. \citep{caldas2015object} transform a manipulation control problem with contact to uncertainties to a standard optimization problem with linear matrix inequalities (LMI), tuning an impedance control scheme to robust manipulation.




==> ML.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% read about meta-learning and one-shot, zero, others
% student teacher
% curriculum learning

The establishment of control policies for in-hand manipulation remains challenging regardless of gripper, object or task properties. Various contact models and hand configurations have been used in the literature to develop kinematic and dynamic models for in-hand manipulation as described in previous sections. In order to execute in-hand manipulation tasks with these models, detailed knowledge of the object-hand interaction is required. For most robotics scenarios, however, such information cannot be reasonably estimated using conventional analytical methods since precise object properties are often not a priori known. 
%Sensory information, if available, is usually noisy. 
Model learning offers an alternative to careful analytical modeling and accurate measurements for this type of system, either through robot interaction with the environment or human demonstrations. Learning a model can be done explicitly using various Supervised Learning (SL) techniques, or implicitly by maximizing an objective function. In this section, we will focus on the former technique of supervised learning while the latter will be covered in the following section.

% ------------------------------------------------

\subsection{Learning state representation} 

Learning a state representation for in-hand robotic manipulations refers to the process of developing a mathematical model that describes the various states of the hand-object system during manipulation. This model can be used to represent the position, orientation, velocity, and other physical properties of an object. Furthermore, the model can be used to predict object response to certain actions. 

State representation is an important building block where the object-hand configuration is sufficiently described at any given time. For example, if a robot is trying to roll an object within the hand, it may use some state representation to measure and track the object's pose, and use this information to exert informed actions. In SL, an ANN is commonly used to extract relevant features from data and learn useful features from high-dimensional observation spaces \citep{azulay2022learning, andrychowicz2020learning, Funabashi2019,Sodhi2020,Dimou2023}. It is also effective in combining data from multiple sensors or information sources \citep{qi2022}, and is often used by robots to merge information from different modalities, such as vision and haptic feedback \citep{andrychowicz2020learning}. Without a compact and meaningful representation of the object-hand state, the robot may struggle to perform successful and efficient manipulations \citep{azulay2022learning}.

Haptic perception is commonly used to learn various features of an object in uncertain environments so as to grasp and manipulate it. Such information may include stiffness, texture, temperature variations and surface modeling \citep{Su2012}. Often, haptic perception is used alongside vision to refine initial pose estimation \citep{Bimbo2013}. Contact sensing is the common approach for pose estimation during manipulation \citep{azulay2022learning}. Such sensing has been generally achieved using simple force or pressure sensors \citep{Tegin2005, cheng2009novel, wettels2009multi}. As such, \cite{Koval2013} used contact sensors and particle filtering to estimate the pose of an object during contact manipulation. \cite{Park2024} used soft sensors in a pneumatic finger and a neural-network to estimate the angles of the finger. In recent years, optical sensor arrays have become more common due to advancements in fabrication abilities and due to their effectiveness in covering large contact areas \citep{Bimbo2016}. The softness of the sensing surface allows the detection of contact regions as it deforms while complying with the surface of the object. Changes in images captured by an internal camera during contact are analyzed. 

Several works have used data from optical-based tactile sensors and advanced deep-learning networks to estimate the relative pose of an object during contact manipulation. For example, \cite{Sodhi2020} used data from an optical-based tactile sensor to estimate the pose of an object being pushed, while others \citep{Lepora2020, psomopoulou2021robust} explored the use of these sensors for estimating the relative pose of an object during a grasp. In a work by \cite{wang2020swingbot}, the use of tactile sensing for in-hand physical feature exploration was also explored in order to achieve accurate dynamic pivoting manipulations. \cite{wang2020swingbot} also used optical tactile sensors on a parallel gripper in order to train a model to predict future pivoting angles given some control parameters. \cite{Toskov2023} addressed the pivoting with tactile sensing and trained a recursive ANN for estimating the state of the swinging object. The model was then integrated with the gripper controller in order to regulate the gripper-object angle. \cite{Funabashi2019} learned robot hand-grasping postures for objects with tactile feedback enabling manipulation of objects of various sizes and shapes. These works demonstrate the potential of haptic perception and learning techniques for improving the accuracy and efficiency of in-hand manipulation tasks. In practice, tactile sensing provides valuable state information which is hard to extract with alternative methods. %Evidently, since 20?? the number of papers has grown by ??\% compared to the previous decade. 



% ------------------------------------------------

\subsection{Learning hand transition models}
\label{sec:transition_model}

A common solution for coping with the unavailability of a feasible model is to learn a \textit{transition model} from data. Robot learning problems can typically be formulated as a Markov Decision Process (MDP) \citep{Bellman1957}. Hence, a \textit{transition model}, or \textit{forward model}, is a mapping from a given state $\ve{x}_t\in\ssl{X}$ and action $\ve{a}_t\in\ssl{A}$ to the next state $\ve{x}_{t+1}$, such that $\ve{x}_{t+1} = f(\ve{x}_t,\ve{a}_t)$. Subsets $\ssl{X}$ and $\ssl{A}$ are the state and action spaces of the system, respectively. Such models are commonly obtained through non-linear regression in a high-dimensional space. Often, the forward model is described as a probability distribution function, i.e.,  $P(\ve{x}_{t+1}|\ve{x}_t,\ve{a}_t)$, in order to represent uncertainties in the transition.

Learning transition models for in-hand manipulation tasks typically involves understanding how changes in the robot's state are caused by its actions \citep{nagabandi2020deep}. While a hand transition model is generally available analytically in rigid hands where the kinematics are known \citep{Ozawa2005}, analytical solutions are rarely available for compliant or soft hands. As far as the authors' knowledge, the major work on learning transition models involves such hands. %Hence, the authors have not found work concerning learning of a model for rigid hands in the context of in-hand manipulation.
Attempts to model compliant hands usually rely on external visual feedback. For example, \cite{Sintov2019} proposed a data-based transition model for in-grasp manipulation with a compliant hand where the state of the hand involves kinesthetic features such as actuator torques and angles along with the position of the manipulated object acquired with visual feedback. The extension of this work used a data-based transition model in an asymptotically optimal motion planning framework in the space of state distributions, i.e., in the belief space \citep{kimmel2019belief,sintov2020motion}. Recently, \cite{morgan2020object} proposed an object-agnostic manipulation using a vision-based Model Predictive Control (MPC) by learning the manipulation model of a compliant hand through an energy-based perspective \citep{morgan2019data}. The work by \cite{Wen2020} used a depth camera to estimate the pose of an object grasped and partly occluded by the two fingers of an underactuated hand. While the work did not consider manipulation, an extension proposed the use of the depth-based 6D pose estimation to control precise manipulation of a grasped object \citep{Morgan2021}. The authors leverage the mechanical compliance of a 3-fingered underactuated hand and utilize an object-agnostic offline model of the hand and the 6D pose tracker using synthetic data. 
While not strictly a transition model, \cite{Calli2018} trained a model to classify transitions and identify specific modes during in-grasp manipulations of an underactuated hand. By using visual and kinesthetic perception, state and future actions are classified to possible modes such as object sliding and potential drop.

% Avishai: No learning here
%Moreover, Morgan et al. \citep{morgan2022complex}, also introduced a method that achieves complete $SO(3)$ finger gaiting control of grasped objects against gravity by developing a manipulation planner that operates via orthogonal safe modes of an underactuated hand absent of tactile sensors or joint encoder.

While the above methods focus on pure visual perception for object pose estimation, tactile sensors were used in recent work independently or combined with vision. Recent work integrated allocentric visual perception along with four tactile modules, that combine pressure, magnetic, angular velocity and gravity sensors, on two underactuated fingers \citep{Fonseca2019}. These sensors were used to train a pose estimation model. \cite{lambeta2020digit} explored a tactile-based transition model for marble manipulation using a self-supervised detector with auto-encoder architectures. \cite{azulay2022learning} tackled the problem of partial or fully occluded in-hand object pose estimation by using an observation model that maps haptic sensing on an underactuated hand to the pose of the grasped object. Moreover, an MPC approach was proposed to manipulate a grasped object to desired goal positions solely based on the predictions of the observation model. A similar forward model with MPC was proposed by \cite{luo2023} for the multi-finger dexterous Allegro hand. Overall, these approaches demonstrate the potential of using external visual feedback fused with tactile sensing to learn transition models for in-hand manipulation tasks of various hands with uncertainty.

% ------------------------------------------------

\subsection{Self-supervision and Exploration for Learning Transitions} 

Self-supervision and exploration are important techniques for learning transitions of in-hand robotic manipulation. Self-supervision refers to the process of learning from unlabeled data, where the learning algorithm is able to infer the desired behavior from the structure of the data itself. This can be particularly useful for in-hand manipulation, as it allows the robot to learn about the various states and transitions of an object without the need for explicit human supervision. Exploration, on the other hand, refers to the process of actively seeking out and interacting with the environment in order to collect useful data. In the context of in-hand manipulation, exploration can involve the robot trying out different grasping and manipulation strategies in order to learn what works best for a given object and task. By actively seeking out and interacting with the environment in this way, the robot can learn about the various states and transitions of the object through trial and error, and utilize this knowledge to improve its manipulation performance. Together, self-supervision and exploration can be powerful tools for learning transitions in in-hand manipulation, as they allow the robot to learn from its own experiences and actively gather information about the object being manipulated and its surroundings.

The collection process to generate a state transition model for a robotic system requires active exploration of the high-dimensional state space \citep{kroemer2021}. The common strategy is to exert random actions \citep{calli2018path} in the hope of achieving sufficient and uniform coverage of the robot's state space. In practice, some regions are not frequently visited and consequentially sparse. In systems such as compliant hands \citep{SintovL4DC2020} or object throwing \citep{Zeng2020}, each collection episode starts approximately from the same state and, thus, data is dense around the start state while sparser farther away. Therefore, acquiring state transition models for robotic systems requires exhausting and tedious data collection along with system wear, i.e., the transition function $f(\ve{x}_t,\ve{a}_t)$ is difficult to evaluate.

Active sampling is an alternative strategy where actions that are more informative for a specific task are taken \citep{Wang2018}. However, acquiring a general model of the robot requires the exploration of the entire feasible state space. Bayesian Optimization is the appropriate tool to identify key locations for sampling that would provide increased model accuracy. However, having knowledge of sampling locations does not guarantee the ability to easily reach them. Reaching some state-space regions may require exerting complicated maneuvers. The right actions that will drive the system to these regions for further exploration are usually unknown, particularly in preliminary stages with insufficient data. That is, we require a good model in order to learn a good model.




% Different machine learning approaches have been followed to control robotic hands \citep{YanyuSu2013, Levine2015}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% adaptive hands transition modeling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%% NOT CITED

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9938409

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tactile based
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \citep{ward2017model} -  demonstrate in-hand reorientation of grasped objects through active tactile manipulation. object location is actively controlled based on the classification results of incoming tactile data

% \citep{paolini2016data} data-driven statistical modeling (kernel density estimation) of cube re-grasping with rigid hand  For instance, the use of GP for cube re-grasping with rigid hand is explored in 

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9812212
% https://arxiv.org/pdf/2204.03698.pdf
% https://arxiv.org/pdf/2201.11503.pdf
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9691924
% https://proceedings.mlr.press/v164/chen22a/chen22a.pdf
% https://arxiv.org/pdf/2210.04887.pdf
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9762182

==> RL.tex <==

Reinforcement learning (RL) is one of the main paradigms of machine learning, akin to supervised and unsupervised learning. RL models learn to take optimal actions within some environments by maximizing a given reward (Figure \ref{fig:RL1}). In contrast to model-driven learning, most RL algorithms collect data during the learning process. Often, the learning is done in simulated environments in order to avoid tedious work and wear of the real robot. RL policies are functions mapping current states to optimal actions and a distinction is commonly made between on- and off-policy learning \citep{Singh2022}. Both approaches commonly approximate the value function which is an expected cumulative reward defined for states and actions. In on-policy learning, data collection is guided by the intermediate policy learned by the agent. The value function is learned directly by the policy. 
Therefore, a balance must be kept between exploration of unvisited action-state regions, and exploitation of known regions in order to maximize reward. In off-policy methods, on the other hand, the value function of the optimal policy is learned independent of the actions conducted by the agent during training. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/RLdiagram.png} 
    \caption{Illustration of (left) basic RL, (top right) actor-critic architecture, and (bottom right) a multi-network architecture.}
    \label{fig:RL1}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ---------------------------------------------------

\subsection{Formal RL Definition}

%%%%%%% Formal RL paragraph %%%%%
We briefly present the formal definition of RL. A wider review of key concepts and methods can be found in the work of \cite{Nguyen2019}. Assuming that a given system is a Markov Decision Process (MDP), the system can be defined by the tuple $\{\mathcal{S,A},P,\mathcal{R},\delta\}$ where $\mathcal{S}$ and $\mathcal{A}$ are the state and action spaces, respectively. In MDP, the next state depends solely on the current state $\ve{s}_t\in\mathcal{S}$ and desired action $\ve{a}_t\in\mathcal{A}$ according to a forward transition dynamics $P(\ve{s}_{t+1}|\ve{s}_t, \ve{a}_t)$ while receiving a reward ${r_t}\in\mathcal{R}$. Scalar $\delta>0$ is the discount factor which reflects the significance of the reward over time. In model-based RL, transition model $P$ can be learned independently of the policy learning as described in Section \ref{sec:transition_model}. 

When the system is stochastic due to uncertainties and limited observability, a Partial Observed Markov Decision Process (POMDP) is considered. The POMDP can be defined by the tuple $\{\mathcal{S,A,O},P,\mathcal{Z,R}, \delta\}$, where $\mathcal{S}$ is now the unobserved state space and $\mathcal{O}$ is the observation space. As the true state cannot be fully observed, an observation space $\mathcal{O}$ is introduced to describe the set of all possible observations. Therefore, the agent receives an observation  $\ve{o}_{t+1}\in\mathcal{O}$ when reaching the next state $\ve{s}_{t+1}$ with probability $\mathcal{Z}(\ve{o}_{t+1}|\ve{s}_{t+1})$. In both MDP and POMDP, the goal is, therefore, to learn a policy $\ve{\pi}:\mathcal{S}\to\mathcal{A}$ or $\ve{\pi}:\mathcal{O}\to\mathcal{A}$, respectively, which maximizes the expected reward $\mathbb{E}\left\{\sum_{t=0}^{H}\delta^{t}r_t\right\}$, where $H\in\mathbb{R}^+$ is the horizon. By modeling the system as a POMDP and using RL, the agent has the potential to minimize the true error within a sequence of actions rather than applying greedy ones, such as in supervised learning policies. 

%find first definition of NN and use NN since then. same with deep=D. seems this term is not currently introduced earlier, except in specific examples. Should probably appear in an earlier section's introductory part.
Deep reinforcement learning integrates the RL learning paradigm with deep ANNs serving as the policy or value function approximation. Such integration has revealed significant capabilities and led to the success of many reinforcement learning domains \citep{mnih2013playing,mnih2015human} including robot manipulation \citep{levine2016end,Nguyen2019} and specifically in-hand dexterous manipulation \citep{Jain2019,andrychowicz2020learning}. Examples of straight-forward implementation of an RL algorithm include the work of \cite{antonova2017reinforcement} which addressed the pivoting problem with a parallel gripper. The RL policy was trained while relying on fast tracking with a camera. However, the trained policy yielded excessive back and forth motions. \cite{Cruciani2017} coped with this limitation by employing a three-stage manipulation in which the robot learns to control the velocity and opening of the gripper. An RL policy was acquired through Q-Learning \citep{watkins1992q}. In an extension work, \cite{Cruciani2018} integrated path planning with the RL policy for the robotic arm to perform more complex tasks. In another example, \cite{VanHoof2015} was the first to employ RL on a two-finger underactuated hand by utilizing its compliance and tactile sensing. 

Direct implementation of RL algorithms usually only works in specific and limited applications. Hence, this section presents a comprehensive survey of advanced approaches and current research in the field, with a focus on the unique challenges of in-hand manipulation. First, we describe transfer learning challenges and approaches focusing on the \sr problem. Next, the problem of episodic resetting in real-life experiments is discussed. Finally, we explore the topic of multi-level control systems and actor-critic learning schemes.  

% ---------------------------------------------------

\subsection{Transfer learning and \sr problems}

Often, ANN based controllers must train extensively for each new task before being able to perform successfully, requiring long training periods and extensive computation resources. Specifically for in-hand manipulation, performing tasks with trained policies on new objects may be challenging. Transfer learning can be divided into few-shot, one-shot and zero-shot learning \citep{Pourpanah2023}. Few-shot and one-shot transfer learning requires few instances or a single instance, respectively, of a new task in order to tune the previously trained model. On the other hand, a trained model in zero-shot transfer can instantly perform tasks not included in the training stage. Thus, the ability to learn and generalize to new tasks in few-shots or less is highly beneficial. In in-hand manipulation, the transfer of a model often refers to the generalization to new objects not included in the training \citep{Huang2021}.

The common approach in few- and one-shot transfer learning is to share weights and data between different tasks, objects and hands. \cite{funabashi2019morphology} demonstrated the ability to pre-train a policy to perform a stable rolling motion with only three fingers of the Allegro hand and then transfer to utilize all four fingers. This was shown to be possible given identical finger morphologies. It was shown that pre-training can be done with data gathered even from random motions such that, afterward, training for specific tasks can be done in one-shot transfer. 

%add short connecting sentence
While training RL models on real robots yields highly successful controllers \citep{kalashnikov2018scalable,zhu2019dexterous}, it is also expensive in time and resources, or can pose danger with some robots. Furthermore, it tends to require extensive human involvement as discussed in the next section.
%Training on real robots is expensive in time and resources and requires extensive human involvement as further discussed in the next section. On the other hand, sufficient data collection yields highly successful controllers \citep{kalashnikov2018scalable,zhu2019dexterous}. 
Consequently, simulations are an emerging approach for policy training as they enable rapid and efficient collection of a massive amount of data. While training on simulations can be beneficial, transferring a robot policy trained in simulation to a real robot remains a challenge \citep{zhao2020sim}. Compared to real-world systems that are usually uncertain and noisy, simulations are naturally more certain and simplified. This gap is commonly known as the \sr problem and can significantly reduce the performance of policies trained in the simulation domain and transferred to the application domain in the real world \citep{hofer2021sim2real}. This is especially relevant in the case of in-hand manipulation tasks which tend to heavily involve hard-to-model contact dynamics \citep{funabashi2020variable,liarokapis2016post}. Hence, the resulting controllers are often sensitive to small errors and external disturbances. 

The most common approach for bridging the reality gap in a \sr problem is \textit{domain randomization} \citep{van2019sim}. In this approach, various system parameters in the simulation are constantly varied in order to improve robustness to modeling errors. \cite{OpenAI2019,andrychowicz2020learning} proposed the Automatic Domain Randomization (ADR) approach where models are trained only in simulation and can be used to solve real-world robot manipulation problems. Specifically, a Rubik's cube was solved by performing finger gaiting and rolling manipulations with the anthropomorphic Shadow hand. ADR automatically generates a distribution over randomized environments. Control policies and vision state estimators trained with ADR exhibit vastly improved \sr transfer. %For control policies, memory-augmented models trained on an ADR-generated distribution of environments show clear signs of emergent meta-learning at test time. 

In the work of \cite{Sievers2022}, a PyBullet simulation of the DLR hand was used to train an off-policy for in-grasp manipulation solely using tactile and kinesthetic sensing. Domain randomization was used for \sr transfer to the real hand. An extension of the work has demonstrated zero-shot \sr transfer while focusing on 24 goal orientations \citep{Pitz2023}. Beyond directly modifying the dynamics in domain randomization, applying small random forces to the grasped object was shown by \cite{allshire2022transferring} to improve the robustness of the resulting policy in in-grasp manipulation of the TriFinger hand. Recently, \cite{Handa2023} have taken the domain randomization approach to reorient a cube within the four-finger Allegro hand using RGB-D perception. As opposed to Pybullet and similar simulators which are based on CPU computations, \citeauthor{allshire2022transferring} and \citeauthor{Handa2023} used the GPU-based Nvidia Isaac Gym simulator \citep{makoviychuk2021isaac}. Using a GPU-based simulator reduces the amount of computational resources and costs. 

As opposed to domain randomization, \cite{qi2022} used an adaptation module learning to cope with the \sr problem. The module trained through supervised learning to approximate the important properties of the system based solely on kinesthetic sensing. An RL policy is trained to take actions for finger gaiting with a multi-finger hand based on the approximations and on real-time state observations. An extension of the work added visual and tactile perception while also including a Transformer model for embedding past signals \citep{Qi2023}. \citeauthor{Qi2023} have also used the Isaac Gym simulator since it excels in contact modeling. However, Isaac Gym and most other simulators tend to provide unreliable contact force values. To cope with this limitation, \cite{Yin2023} simulated 16 tactile sensors across a four-finger Allegro (i.e., fingertips, fingers and palm) while considering only binary signals of contact or no contact. Due to this configuration, a trained policy is shown to successfully ease the \sr transfer.



% Avishai: the citation is not correct and I cannot track the relevant one
% Another avenue for improving the accuracy of the simulator is modeling specific aspects of reality such as mimicking sensor faults and camera frame latency \citep{allshire2022transferring}. 

% Avishai: These are not relevant to in-hand manipulation or RL
% Jianu et al. \citep{jianu2022reducing} addressed the \sr problem of optical tactile sensors by training a generative model to map simulated tactile images to photorealistic ones. 
% RL policies with such simulated tactile sensing were shown to learn object pose estimation more successfully \citep{zhao2022skill}. Such property is highly important for in-hand manipulation. 

% ---------------------------------------------------

\subsection{Episodic resetting}

Learning robot tasks in the real world often requires sufficient experience. In many systems, this is commonly achieved with frequent human intervention for resetting the environment in between repeating episodes, for example when the manipulated object is accidentally dropped. It is particularly relevant in the case of in-hand manipulation where resetting may be more complex due to large uncertainties in failure outcomes. Removing the costly human intervention will improve sample collection and, thus, decrease learning time. \cite{eysenbach2018leave} proposed a general approach for training a reset policy simultaneously with the task policy. For instance, a robot manipulator can be trained to reset the environment within the policy training allowing a more autonomous and continuous learning process. As shown by \cite{srinivasan2020learning}, the resulting reset policy can be used as a critic for the task controller in order to discern unsafe task actions that will lead to irreversible states, where reset is inevitable. Specifically in this work, a model learns to identify actions that a Shadow hand may exert while attempting to reorient a cube through rolling and finger gaiting, without the risk of dropping the cube entirely. Preventing the reach of these irreversible states increases the safety of the controller, and can also be used to induce a curriculum for the forward controller. 

Another approach to avoid irreversible states is by the addition of a reactive controller designed specifically for intervening only when the robot state is in the close neighborhood of such irreversible states \citep{Falco2018}. In this work, \citeauthor{Falco2018} used a compliant prosthetic hand in the in-grasp manipulation of objects based on visual perception with an added reactive controller connected to tactile sensors. The goal of the reactive controller is to avoid object slipping. The nominal control method can, thus, be trained with the goal of not only succeeding in the given task but also minimizing the intervention of the reactive controller.

While episodic resetting is often considered a burden, it can instead be considered an opportunity. When training multi-task capabilities for in-hand manipulation, failure in one task may cause a need for a resetting of the grasp. Rather than using human intervention or an additional control system, the reset can instead be viewed as another manipulation task \citep{Gupta2021}. For example, an unsuccessful attempt at a rolling motion %using a four-finger dexterous hand, 
which leads to a wrong object pose, may require the learning of a sliding task to fix the pose. Thus, task training ending in success or failure can both be chained to further learning of other tasks. This results in a reset-free learning scheme.

% ---------------------------------------------------

\subsection{Multi-network architecture} 

Multi-network architectures, such as actor-critic \citep{lillicrap2015continuous} or teacher-student \citep{zimmer2014teacher}, are often beneficial in improving the learning process. In the more common actor-critic structure, an actor network is trained as the policy while the critic network is trained to estimate the value function. Such structures try to cope with the inherent weaknesses of single-network structures. That is, actor-only models tend to yield high variance and convergence issues while critic-only models have a discretized action space and, therefore, cannot converge to the true optimal policy. In teacher-student architectures, on the other hand, knowledge distillation enables the transfer of knowledge from an unwieldy and complex model to a smaller one. As such, a teacher model is an expert agent that has already learned to take optimal actions whereas the student model is a novice agent learning to make optimal decisions with the guidance of the teacher. %The distillation notion originates from the use of human experts teaching but was extended to include the use of expert ANNs.

\cite{chen2021simple, chen2022,Chen2023} used an asymmetric teacher-student training scheme with a teacher trained on full and privileged state information. Then, the teacher policy is distilled into a student policy which acts only based on limited and realistic available information. Policies for object reorientation tasks were trained with a simulated Shadow hand on either the EGAD \citep{morrison2020egad} or the YCB \citep{calli2015ycb} benchmark object sets and tested on the other. Results have exhibited zero-shot transfer to new objects. While the teacher-student approach utilizes privileged information during training, the actor-critic approach manages the learning by continuous interaction between the two models. This was demonstrated with the Proximal Policy Optimization (PPO) algorithm for in-hand pivoting of a rigid body held in a parallel gripper, using inertial forces to facilitate the relative motion \citep{Toledo2021}. Moreover, combining actor-critic methods with model-based methods can result in improved learning. The learned model can be used within a model predictive controller to reduce model bias induced by the collected data. This was demonstrated by an underactuated hand to perform finger gaiting \citep{morgan2021model} and object insertion \citep{azulay2022haptic}. Recently, \cite{Tao2023} proposed to consider the multi-finger hand during a reorientation task as a multi-agent system where each finger or palm is an agent. Each agent has an actor-critic architecture while only the critic has a global observation of all agents. The actor, on the other hand, has only local observability of neighboring agents. In such a way, the hand does not have centralized control and can adapt to changes or malfunctions.

In a different multi-modal architecture approach proposed by \cite{Li2020}, various control tasks required for in-hand manipulation are divided into multiple hierarchical control levels (Figure \ref{fig:RL1}). This allows the use of more specialized tools for each task. In the lower level, traditional model-based controllers robustly execute different manipulation primitives. On the higher level, a learned policy orchestrates between these primitives for a three-finger hand to robustly reorient grasped objects in a planar environment with gravity. A similar approach was taken by \cite{Veiga2020} where low-level controllers maintain a stable grasp using tactile feedback. At the higher level, an RL is trained to perform in-grasp manipulation with a multi-finger dexterous hand.

% ---------------------------------------------------

\subsection{Curriculum Learning}

Often, directly training models with data from the entire distribution may yield insufficient performance. Hence, Curriculum Learning (CL) is a training strategy where the model is gradually exposed to increasing task difficulty for enhanced learning efficacy \citep{wang2021survey}. Such a process imitates the meaningful learning order in human curricula. Adding CL to guide the development of necessary skills can aid policies to learn difficult tasks that tend to have high rates of failure \citep{chen2022}. In this example, researchers modify the behavior of gravity in simulations according to the success rate to aid the learning of gravity-dependent manipulation tasks. This method allows the robot to first successfully learn a skill and then move on to increasingly harder and more accurate problems, slowly reaching the actual desired skill. \cite{azulay2022haptic} trained an actor-critic model to insert objects into shaped holes while performing in-grasp manipulations with a compliant hand. The work has exhibited object-based CL where simple objects were first introduced to the robot followed by more complex ones. Other uses of CL can involve guiding the exploration stages of solution search using reward shaping \citep{allshire2022transferring}. The work shows that it is possible to improve early exploration by guiding the model directly to specific regions using specific reward functions as priors. Those regions however may not hold actual feasible solutions, and it may be necessary to reduce the effects of the reward functions in later stages of the learning process. 

% ---------------------------------------------------

\subsection{Tactile information}

While visual perception is a prominent approach for feedback in RL, it may be quite limited in various environments and the object is often occluded by the hand. On the other hand, tactile sensing provides direct access to information regarding the state of the object. Nevertheless, data from tactile sensing is often ambiguous, and information regarding the object is implicit. Yet, the addition of tactile sensory is widely addressed as it can improve the learning rate. For instance, in the work of \cite{korthals2019multisensory}, tactile sensory information for the Shadow hand increased the sampling efficiency and accelerated the learning process such that the number of epochs for similar performance was significantly decreased. 
% Another benefit of tactile sensing is emphasized when the hand occludes line-of-sight of the camera to the object as may commonly occur during in-hand manipulation tasks. 
\cite{Jain2019} have shown that the integration of tactile sensors increases the learning rate when the object is highly occluded. This was demonstrated in various manipulation tasks including in-hand manipulation of a pen by a simulated anthropomorphic hand. \cite{melnik2019tactile} compared multiple sensory methods, including continuous versus binary (i.e., touch or no touch) tactile signals and, higher versus lower sensory resolutions. The results from this comparative study have shown that using tactile information is beneficial to the learning process, compared to not having such information. However, the specific method that gave the best result was dependent on the learned manipulation task \citep{melnik2021}. 

While \citeauthor{melnik2021} used tactile information directly as part of the state vector, \cite{funabashi2020variable,funabashi2020stable} used a higher-resolution sensory array without visual perception. The model coped with the increased dimension of the output tactile information by considering the relative spatial positioning of the sensors. Similarly, \cite{Yang2023} used a tactile array across a multi-finger hand. The array was embedded using Graph Neural Network which provides an object state during the manipulation and used for model-free RL. Recently, \cite{Khandate2022} implemented model-free RL to reorient an object through finger gaiting with a multi-finger dexterous hand while only using kinesthetic and tactile sensing. In an extension work, \citeauthor{Khandate2022} offered the use of sampling-based motion planning in order to sample useful parts of the manipulation space and improve the exploration \citep{Khandate2023}. Tactile sensing provides valuable information and often can fully replace visual perception. However, policies based on tactile perception usually require an excessive amount of real-world experience in order to reach sufficient and generalized performance.

\hfill

In summary, research in the field of RL for robotic in-hand manipulation is growing and achieving increasing success in recent years.  While showcasing promising performance in specific tasks, RL policies still perform poorly in multi-task scenarios and struggle to generalize with zero- or few-shot learning \citep{Chen2023bi}. Major challenges currently being faced include the control of highly dexterous hands with high amounts of sensory information, the transfer of a model learned in simulation to a real robotic system, and the transfer of learning specific tasks on well-known objects to other tasks and unknown objects. Major advances are being achieved using multi-level control structures, domain and dynamic adaptation, and the combination of model-based and model-free methods to gain the benefits of both. While exciting advances have been made in RL, the field continues to explore the challenges of data efficiency and adaptability to new domains. 


%add a sentence on decision transformers.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% this section now seems connected to no specific part, would appreciate advice on where to place it.
  % Another way to construct a multi-level controller is to separate the tasks of choosing the action and predicting its result \citep{nagabandi2020deep}. A neural network can serve as a predictor of the future states of the system by learning its dynamics. An iterative algorithm can then use the predictor to simulate the results of possible actions at each step and converge to approximately optimal trajectories.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> abstract.tex <==
\begin{abstract}
Human dexterity is an invaluable capability for precise manipulation of objects in complex tasks. The capability of robots to similarly grasp and perform in-hand manipulation of objects is critical for their use in the ever changing human environment, and for their ability to replace manpower. In recent decades, significant effort has been put in order to enable in-hand manipulation capabilities to robotic systems. Initial robotic manipulators followed carefully programmed paths, while later attempts provided a solution based on analytical modeling of motion and contact. However, these have failed to provide practical solutions due to inability to cope with complex environments and uncertainties. Therefore, the effort has shifted to learning-based approaches where data is collected from the real world or through a simulation, during repeated attempts to complete various tasks. The vast majority of learning approaches focused on learning data-based models that describe the system to some extent or Reinforcement Learning (RL). RL, in particular, has seen growing interest due to the remarkable ability to generate solutions to problems with minimal human guidance. In this survey paper, we track the developments of learning approaches for in-hand manipulations and, explore the challenges and opportunities. This survey is designed both as an introduction for novices in the field with a glossary of terms as well as a guide of novel advances for advanced practitioners. 

\tiny
 \keyFont{ \section{Keywords:} In-hand manipulation, Dexterous manipulation, Model learning, Reinforcement learning, Imitation learning} %All article types: you may provide up to 8 keywords; at least 5 are mandatory.


% Human dexterity allows for precise and complex manipulation of objects for the completion of tasks. The capability of robots to grasp and manipulate objects is critical for their use in the ever changing human environment, and for their ability to replace human effort. Initial robotic manipulators followed carefully programmed paths, while later research opened the way for more intelligent systems capable of generating grasping solutions and implementing manipulation paths. In recent times, incorporating methods of machine learning has shown increasing success at solving highly complex manipulation problems, and creating manipulators that are robust to errors, disturbances and noise. Reinforcement learning in particular have seen growing interest, due to the enticing ability to generate solutions to problems with minimal need for human guidance. The maturity of the field is shown by recent works incorporating machine learning into increasingly dexterous robot manipulators. The intersection of growth in the fields of dexterous manipulation and machine learning invites an up-to-date survey of the methods of both fields, and how they relate to each other. This work is built around a comprehensive array of taxonomies dividing the topic categories, methods, tasks and challenges. This survey focuses on recent advances in the field, presenting new methods and techniques in humanoid hand design, machine learning, reinforcement learning and imitation learning, as applied to dexterous manipulation. This work also acts as a meta-survey, incorporating analysis of existing surveys of the relevant fields. This survey is designed as a both an introduction for novices in the field, as well as a guide for novel advances for veteran researchers. 
\end{abstract}

==> disc.tex <==
% \subsection{osher's part}

In-hand manipulation is one of the most challenging topics in robotics and an important aspect for feasible robotic applications. Traditional analytical methods struggle to estimate object properties and noisy sensory information. With in-hand manipulation reaching a bottleneck using these traditional methods, researchers are leveraging advancements in deep learning and reinforcement learning to unlock new levels of dexterity. These tools encapsulate the ability to model complex and noisy systems such as a dexterous robotic hand equipped with various sensors. Nevertheless, current research still faces significant challenges:

\begin{enumerate}
    \item \textit{Data efficiency.} Learning models is essential for understanding changes in the robot's state caused by its actions during in-hand manipulation. While analytical solutions are available for rigid hands, compliant or soft hands rely on external visual feedback. However, collecting data can be challenging due to the high-dimensional state space and the need to explore the entire feasible space. Future work by researchers should address methods to reduce the required size of training data by making models more general to various applications. For instance, Bayesian optimization can assist in identifying key sampling locations, but reaching some regions may require complex maneuvers, making it necessary to have a good prior model to learn a better one.
    
    \item \textit{Sim-to-real transfer.} Learning policies in simulation is a prominent approach to improve data efficiency in robot training. While significant progress has been made to address the \sr problem, simulations hardly represent the real world and trained policies work poorly on the real system. Hence, large efforts should be put into closing the reality gap by generating better simulations and, incorporating advanced data-based models that can generalize better. Examples of the latter include decision transformers \citep{Monastirsky2023} and diffusion policies \citep{chi2023diffusionpolicy}.

    \item \textit{Soft robotic hands.} High-dexterous hands such as anthropomorphic ones have been demonstrated in multiple complex in-hand manipulation tasks. However, they are highly expensive making their adaptation to real-world tasks not possible. Consequently, an abundance of research and development has been put in recent years on soft robotic hands that are typically low-cost to manufacture. However, these hands cannot be modeled or controlled analytically and learning approaches are the common paradigm. As discussed previously, common solutions require a significant amount of data and are usually specific to a single hand and task. Therefore, the robotics community should promote efficient learning approaches that can be generalized to different hardware, tasks and environments.
    
    \item \textit{Tactile sensing.} While visual perception technology is quite mature, the use of high-resolution tactile sensing is relatively new. In general, Table \ref{tb:Pcomparison} clearly shows the dominance of visual perception over tactile sensing in research. Highly capable tactile sensors can provide vital information regarding the contact state including position, forces, torsion, shape and texture. Nevertheless, they often require a large amount of real-world data in order to perform well. Simulations such as TACTO \citep{wang2022tacto} address this problem by simulating tactile interactions. However, these remain quite far from reality and cannot provide reliable load sensing. Practitioners should work toward better tactile simulators along with distillation approaches for efficient \sr transfer.

    \item \textit{Learning from Demonstrations.} IL with expert demonstrations has proved to be efficient for shortening the data-hungry training phase of RL. However, hardware and methods for collecting demonstration data generally lack the ability to capture the entire state space of the hand-object system. For instance, visual perception is incapable of observing the intrinsic and contact state of the system. Furthermore, IL models focus on task completion and fail to address strategy learning with efficient data utilization. Future work should facilitate efficient platforms for collecting high-dimensional data in the real world. In addition, learning methods should require a small amount of data from the expert user in order to generalize well to various scenarios of the tasks. 

    \item \textit{Task generalization.} The prevailing paradigm in in-hand manipulation focuses on crafting task-specific or narrowly applicable policies, which hinders broader applicability. The field therefore necessitates a paradigm shift toward solutions capable of seamless adaptation or generalization to novel tasks or objects.
\end{enumerate}


% Control policies for in-hand manipulation face challenges in modeling and controlling of various grippers, objects and tasks. Traditional analytical methods struggle to estimate object properties and sensory information is often noisy. Model learning techniques offer an alternative by leveraging robot-environment interaction or human demonstrations. Supervised learning, particularly using NN, has proven effective in extracting features from high-dimensional observation spaces and merging data from multiple sensors. A compact and meaningful state representation of the hand-object system is crucial for successful manipulations, with haptic perception providing valuable information that is difficult to extract using other methods.

Overall, learning approaches such as supervised learning, haptic perception and self-supervision, along with the combination of visual and tactile sensing, show promise in enhancing the accuracy and efficiency of in-hand robotic manipulation tasks. These techniques enable robots to acquire a comprehensive understanding of the object-hand system and improve their manipulation capabilities. Many challenges remain to be met by the academic community in order for high-ability robots to be used in real-world applications.



==> introduction.tex <==

%The field of robot in-hand manipulation has long been considered a challenging one. Yet, it has seen rapid development in recent years. With the vast industrial development as well as increase in demand for domestic usage, a significant growth of interest in this field can be predicted. Evidently, we witness the increase in research papers, as seen in Figure \ref{fig:stats}, along with algorithms for solving versatile tasks. Just to mention a few, there are tasks such as welding, medical procedures, assembly and robotic assistance to sick and disabled users. In times of pandemic, we have witnessed the significant need for using autonomous and complex robot manipulations \citep{kroemer2021}. 

%In this paper, we survey the various in-hand manipulation tasks of robotic hands and the advanced learning approaches for achieving them. As commonly done by the robotics community and as seen in Figure \ref{fig:InHandTaxonmy}, we make a distinction between two main categories of robot in-hand manipulation: \textit{dexterous} and \textit{non-dexterous} in-hand manipulations. To the best of our research, we can conclude that the former approach is more proliferated from algorithms and number of published papers perspective. In addition, we divide the manipulation approaches into continuous and non-continuous techniques. We can also see in Figure ~\ref{fig:InHandTaxonmy} that the continuous approach has more techniques than the other since continuous approaches include more Degrees Of Freedom (DOF) in comparison to non-continuous ones \citep{sun2021characterizing}.


Robot in-hand manipulation has long been considered challenging. However, it has undergone rapid development in recent years. With the vast industrial development and increase in demand for domestic usage, significant growth in interest in this field can be predicted. Evidently, we witness an increase in research papers, as shown in Figure \ref{fig:stats}, along with algorithms for solving versatile tasks. Just to mention a few, research has sought solutions for real-world tasks such as medical procedures \citep{Lehman2010}, assembly in production lines \citep{kang2021high}, and robotic assistance for sick and disabled users \citep{Petrich2021}. During the COVID-19 pandemic, there has been a significant need for autonomous and complex robot manipulators \citep{kroemer2021}. In this study, we survey various in-hand manipulation tasks of robotic hands and advanced learning approaches for achieving them. As commonly done by the robotics community and as shown in Figure \ref{fig:InHandTaxonmy}, we distinguish between two main categories of robot in-hand manipulation: \textit{dexterous} and \textit{non-dexterous} in-hand manipulations. To the best of our knowledge, we can conclude that the former approach is more prolific in algorithms and the number of published papers. In addition, we divide the types of manipulations into ones that have continuous and non-continuous contacts during execution. The continuous approach has more techniques than the other as it normally uses dexterous robotic hands with higher Degrees-Of-Freedom (DOF) in comparison to non-continuous approaches \citep{sun2021characterizing}.


%In addition, there are more approaches and ways for solving and handling continuous movements tasks than non-continuous. This stem from the fact that real world trajectories are usually continuous \citep{plaku2012planning}.  


%Efforts for learning in-hand manipulation can be classified to three sub-fields: model-based, Reinforcement Learning (RL) and Imitation Learning (IL). Model-based learning focuses on some supervised learning of the dynamics of the system or some state representation. On the other hand, RL is given a reward function which provides a directive for the system to self-learn an optimal policy for completing a task. Similarly, IL requires a policy for imitating human expert demonstration. Figure \ref{fig:stats} shows the increase in paper publications for the three sub-fields over the past five years. In this work, we survey in-hand manipulation approaches, tasks and applications that use either of these sub-fields. 

Efforts for learning in-hand manipulation can be classified into three subfields: model-based methods, Reinforcement Learning (RL) and Imitation Learning (IL). Model-based methods focus on the supervised learning of the dynamics of a system or state representation. On the other hand, RL provides a reward function that embeds an implicit directive for the system to self-learn an optimal policy for completing a task. Similarly, IL requires a policy to imitate human expert demonstrations. Figure \ref{fig:stats} shows the increase in paper publications over the past five years with regard to these three subfields. In this study, we survey in-hand manipulation approaches, tasks and applications that use either of these subfields.  


%To the best of the author's knowledge, this is the first survey of learning approaches for robotic in-hand manipulation. The contribution of this paper is multiple. We map the learning approaches for robot in-hand dexterous manipulation. The papers are classified and grouped into meaningful clusters. The survey can help researchers to efficiently locate relevant research in the right class and perceive what has already been achieved. Practitioners can use our survey for estimating the added value of their research and compare it to previous work. We also explain the relations between the different sub-fields in order to exhibit a wide perspective of the topic. In addition, our work can be seen as a survey of survey papers since some survey papers referred. 

To the best of the author's knowledge, this is the first survey of learning approaches for robotic in-hand manipulation. Hence, this study offers multiple contributions. 
%We map learning approaches for robotic in-hand dexterous manipulation. 
Papers were classified and grouped into meaningful clusters. The survey can help researchers to efficiently locate relevant research in a desired class and perceive what has already been achieved. Table \ref{tb:Pcomparison} provides a summary of prominent state-of-the-art work including key properties. Practitioners can use our survey to estimate the added value of their research and compare it with previous studies. We also explain the relationships between the different subfields to showcase a wide perspective of the topic. In addition, our work can be seen as a survey of survey papers, similar to the references of some other survey papers. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!ht]
%	\begin{center}
%		\includegraphics
%		[scale=0.5]
        %figures/InHandTaxonmy2.png}
%        {figures/Robotic In-Hand Dexterity Manipulation Taxonomy2.png}
%	\end{center}
%	\caption{In Hand Taxonomy (Task Oriented)}
%	\label{fig:InHandTaxonmy}
%\end{figure} 
\begin{figure} 
\centering
\includegraphics[width=\linewidth]{figures/paperstats.png}
\vspace{-0.6cm}
\caption{Statistics on paper publications which addressed or mentioned robotic in-hand manipulations over the past five years in three learning sub-fields: Model-driven learning, Reinforcement Learning (RL) and Imitation Learning (IL), along with papers that do not use any learning method. The search is based on Google Scholar and may include non peer-review publications.}
\label{fig:stats}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!ht]
    \centering
		\includegraphics[width=\textwidth]{figures/inhand.png}
	\caption{Taxonomy of robotic in-hand manipulation.}
	\label{fig:InHandTaxonmy}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%This paper is written in a top-down approach. First, we provide a technical overview on in-hand manipulation including types of manipulations, hands and sensing modalities (Section \ref{sec:Overview}). The overview provides an understanding of relevant hardware, manipulations and common terms to be used later on. Next, we survey the subject from a high-level perspective and later zoom into more detailed sub-topics. We mention the popular tasks in the field. For each task we find the relevant solutions and approaches for solving it. We compare them and find the benefits of one over the other. Finally, we provide insights about future challenges and open problems that should be addressed by the robotics community. 

This study adopts a top-down approach. First, we provide a technical overview of in-hand manipulation, including the types of manipulation, hands and sensing modalities (Section \ref{sec:Overview}). This overview provides an understanding of the relevant hardware, manipulations and common terms to be used later. Next, we survey the subject from a high-level perspective and later zoom into more detailed sub-topics. In addition, we discuss popular tasks in each field. For each task, we often found several approaches while comparing the benefits of one over the other. Finally, we provide insights into future challenges and open problems that should be addressed by the robotics community. 

\input{sum_table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[]
% \centering
% \caption{Feature comparison}
% \label{tb:Fcomparison}
% \begin{tabular}{l|cc|ccccccc|cc|cc}\hline
%                              & \multicolumn{2}{c|}{Dexterity} & \multicolumn{7}{c|}{Type of Manipulation}                                     & \multicolumn{2}{c|}{Hand} & \multicolumn{2}{c}{Perception} \\
%                              & Dex.        & Non-Dex.        & Roll & Pivoting & Sliding & In-Grasp & F. Gait & P\&P & Dyn. & Rigid       & Soft       & Vision        & Haptics        \\\hline
% \multirow{2}{*}{Model-based} &     \citep{Bimbo2013}, \citep{azulay2022learning}        & \citep{Sintov2019,azulay2022learning} &      &          &         & \citep{Sintov2019,azulay2022learning} &         &      &      & &    \citep{Sintov2019,azulay2022learning}         & \citep{Sintov2019}         &   \citep{azulay2022learning}                         \\
%                              &             &                 &      &          &         &          &         &      &      &             &            &               &                \\
% \multirow{2}{*}{RL}          & \citep{Jain2019},\citep{andrychowicz2020learning},\citep{Funabashi2019} ,\citep{qi2022},\citep{azulay2022haptic}               &                 &      &          &         & \citep{Jain2019},\citep{Funabashi2019},\citep{azulay2022learning} ,\citep{azulay2022haptic}         &   \citep{qi2022}       &      &      & \citep{Jain2019},\citep{qi2022},\citep{Funabashi2019}                &            & \citep{Jain2019},\citep{andrychowicz2020learning}               & \citep{Jain2019}  \citep{Funabashi2019},\citep{azulay2022haptic}               \\
%                              &             &                 &      &          &         &          &         &      &      &             &            &               &                \\
% \multirow{2}{*}{IL}          &             &                 &      &          &         &          &         &      &      &             &            &               &                \\
%                              &             &                 &      &          &         &          &         &      &      &             &            &             &\\\hline                 
% \end{tabular}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[]
% \centering
% \caption{Paper comparison}
% \label{tb:Pcomparison}
% \begin{tabular}{lc|ccc|c|c|c|ccc}\hline
% \multicolumn{2}{l|}{\multirow{2}{*}{Paper}} & \multicolumn{3}{c|}{Learning type} & Manipulation type & Dex./Non-Dex. & Rigid/Soft       & \multicolumn{3}{c}{Perception} \\
% \multicolumn{2}{l|}{} & Mod.        & RL       & IL       &      & hand  & hand & Vision   & Tactile   & Kines.  \\\hline

% Sintov et al. & \citep{Sintov2019} & \checkmark & & & In-Grasp & Non-Dex. & Soft & \checkmark & & \checkmark \\
% Andrychowicz et al. & \citep{OpenAI2019,andrychowicz2020learning} & & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark \\
% Jain et al. & \citep{Jain2019} & & \checkmark & \checkmark & In-Grasp & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\
% Funabashi et al. & \citep{funabashi2019morphology,funabashi2020variable,Funabashi2019} & & \checkmark & & Rolling & Dex. & Rigid %with soft fingertips
% & & \checkmark & \checkmark % is the kines. not always true?
% \\
% Allshire et al. & \citep{allshire2022transferring} & & \checkmark &  & In-Grasp & Dex. % edge of dexterity, three dexterous fingers
% & Rigid & \checkmark & & \checkmark
% \\
% Zhao et al. & \citep{zhao2022skill} & & \checkmark & & ?? & Non-Dex. & Rigid & & \checkmark & \checkmark \\
% Srinivasan et al. & \citep{srinivasan2020learning} & & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark \\ %use same environ., robot, and task and nagabandi2019, need to update sensory after adding that paper
% Haozhi et al. & \citep{qi2022} & & \checkmark & & F. Gait. & Dex. & Rigid & &  & \checkmark\\
% Wang et al. &\citep{wang2020swingbot} & & \checkmark & & Dyn. & Non-Dex. & Rigid &  &  & \checkmark \\
% Falco et al. &\citep{Falco2018} & & \checkmark & & In-Grasp & Dex. & Soft & \checkmark & \checkmark & \checkmark \\
% Gupta et al. & \citep{Gupta2021} & & \checkmark & &  Combination & Dex. & Rigid & \checkmark & ? & ? \\ % No info on perception method, likely visual
% Li et al. & \citep{Li2020} & \checkmark & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark \\ % In general I used In-grasp to describe manipulations where it seems the object is grasped during the entire motion, and combination when it is "released" to move dynamically at least for part of the motion.
% % Van-Wyk et al. & 
% % \citep{VanWyk2018}            
% % % &  $\mathbb{R}^{2}$   
% % & \xmark      & \xmark      & \checkmark  & \checkmark   %& \checkmark  
% % &  R\\
% Azulay et al. & \citep{azulay2022haptic, azulay2022learning} & \checkmark& \checkmark & & In-grasp & Non-Dex. & Soft & & \checkmark  & \checkmark\\
% \hline                  

% \end{tabular}


% \end{table*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> overview.tex <==

Robotic in-hand manipulation involves physical interaction between a robotic end-effector, an object and often with the environment. The properties of an end-effector define its ability to manipulate the object including: sensory perception, number of DOF, kinematics and friction. In this section, we provide an overview of various types of in-hand manipulations and the robotic hand types that are capable to exert them. In addition, we discuss the common perception and control methods used in these manipulations.

% -------------------------------------------------------------------

\subsection{Dexterous and non-dexterous manipulation}

The conventional paradigm is to distinguish between dexterous and non-dexterous hands. Generally, dexterous manipulation is the cooperation of multiple robot arms or fingers to manipulate an object \citep{M.Okamura2000}. Dexterous in-hand manipulation is, therefore, the manipulation of an object in the hand by using its own mechanics \citep{Mason1985}. Naturally, dexterous in-hand manipulation requires a high number of DOF and includes, in most cases, anthropomorphic hands. Contrary to dexterous hands, non-dexterous ones have a low number of DOF and, thus, do not have an intrinsic capability to manipulate objects by themselves and require some extrinsic involvement. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.48\linewidth]{figures/jaw_gripper.png} & \includegraphics[width=0.42\linewidth]{figures/allegro.png} \\
    (a) & (b) \\
    \includegraphics[width=0.32\linewidth]{figures/Soft.png} & \includegraphics[width=0.48\linewidth]{figures/uh.png} \\
    (c) & (d) \\
    \end{tabular}
    \caption{Various dexterous and non-dexterous hands. (a) Parallel jaw gripper model 2F-85 by Robotiq. (b) The four-finger Allegro hand with 16 DOF. (c) A four finger soft hand operated by pneumatic bending actuators \citep{Abondance2020}. (d) Underactuated hand model-O from the Yale OpenHand project \citep{Ma2017YaleOP}.}
    \label{fig:hands}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% -------------------------------------------------------------------

\subsection{Types of in-hand manipulations}

We now introduce the types of in-hand manipulations commonly addressed in the literature and distinguish between those that maintain and do not maintain continuous contact with the object. These types can be referred to as both dexterous and non-dexterous manipulations as will be discussed later.

\subsubsection{In-hand manipulations that maintain continuous contact}
Initiating object motion within a robotic hand poses some risk of losing control and potentially dropping it. Hence, the majority of in-hand manipulations perform the motion while maintaining sufficient contact with the object, as it is the safest approach. Nevertheless, a prominent condition for a successful manipulation is that grasp stability is guaranteed throughout the motion. Following are the key in-hand manipulation types that maintain contact.

\begin{itemize}
    
    \item \textit{Rolling.} Rolling manipulation is the ability to rotate an object within the hand through rolling contact. This is caused by finger motion during contact while the object is held against another part of the hand, usually static, such as another finger or palm \citep{Han1997}. Rolling manipulation is limited to objects of certain geometries and is most feasible with round ones. 
    
    \item \textit{Pivoting.} Pivoting is the reorientation of an object between two fingers with respect to the hand \citep{Sintov2016}. The rotation point is commonly the pinching point of the fingers and the reorientation is conducted to some desired angle. The pivoting operation can be done by utilizing gravity \citep{Vina2015}, initiating external contact \citep{Dafle2014} or generating dynamic motions of the robotic arm \citep{SintovSwingUp2016, Cruciani2017}.
    
    \item \textit{Sliding.} In in-hand sliding manipulation, controlled slip is initiated in order to vary the relative position of the object with regards to the hand \citep{shi2017dynamic}. The object slides along the links of the hand to a desired position due to forces from the fingers or external forces \citep{Shi2020}. 
    
    \item \textit{In-Grasp.} While pivoting, sliding and rolling aim to change either position or orientation of the object, in-grasp exploits kinematic redundancy of the hand to vary both the position and orientation of the object \citep{Ma2011}. During manipulation, finger contacts and a stable grasp are maintained. However, sliding or contact rolling may occur \citep{Calli2018}. 
    
    \item \textit{Finger Gaiting.} An approach analogous to gait where the hand’s DOF are exploited to switch between contact locations while maintaining a force-closure grasp \citep{Rus1999,Xu2007,Fan2017}. Hence, the approach is commonly performed quasi-statically where the motion is performed relatively slow to reduce dynamic effects. Finger gaiting may be considered quite wasteful, as it requires sufficiently many DOFs to manipulate the grasped object between two grasp configurations while maintaining stable grasps.  
\end{itemize}

\subsubsection{In-hand manipulations that do not maintain continuous contact}
\begin{itemize}
    
    \item \textit{Pick and place.} While not usually considered as in-hand manipulation, pick-and-place is worth mentioning since it is the most common. The method designates a work area near the robotic arm, where the grasped object can be placed in a controlled manner and then picked up again at a new grasp configuration \citep{Lozano-Perez1987,Tournassoud1987}. This approach consumes valuable production time and occupies a substantial work area.
    
    \item \textit{Dynamic Regrasping.} In this approach, the robot initiates an intended loss of grasp stability through the set of dynamical motions. In most cases,   
    the object is thrown or released into midair and later caught in different grasp configurations. Hence, the hand loses contact (fully or partly) with the object and regains contact by catching it at the final contact points \citep{SintovInHand2017}. Such a method has the advantage of fast manipulation and may require a low number of DOF. However, in contrast to manipulations that maintain contact, the success rate for dynamic regrasping may be lower as object stability is not maintained throughout the motion.
    
\end{itemize}

% -------------------------------------------------------------------

\subsection{In-hand manipulation with Non-dexterous hands}
% Non-dexterous robotic hand - jaw, simple 3 fingers, soft

\subsubsection{Parallel grippers} 

The most common and ubiquitous non-dexterous robotic hand is the \textit{parallel or jaw gripper} seen in Figure \ref{fig:hands}a. Parallel grippers are widely used due to their simplicity, durability and low cost. They can precisely grasp almost any object of the same scale and, therefore, are ubiquitous in industrial applications of material handling \citep{Guo2017}. Parallel grippers normally have only one DOF for opening and closing the jaws. Hence, they do not have independent in-hand manipulation capabilities. Consequently, solutions for in-hand manipulation with parallel grippers often involve the discrete manipulation approach of \textit{pick-and-place} \citep{Tournassoud1987}. In pick-and-place, the object is placed on a surface and picked up again in a different grasp configuration \citep{Zeng2018}. However, the picking and placing can be slow and demands a large surface area around the robot. Hence, approaches for in-hand manipulation with parallel grippers, that do not involve picking and placing, are also divided to \textit{extrinsic and intrinsic dexterity} \citep{Ma2011,Billard2019}. The former compensates for the lack of gripper DOF and involves actions of the entire robotic arm for either pushing the object against an obstacle \citep{Dafle2014,Chavan-Dafle2020} or performing dynamic manipulation. For instance, pivoting can be done by intrinsic slippage control or extrinsic dynamic manipulation of the arm \citep{Vina2015, SintovSwingUp2016, Cruciani2018}. Slippage control leverages gravity and tunes finger contact force of the parallel gripper \citep{Costanzo2021}. \cite{Costanzo2021b} exploited a dual-arm system and tactile feedback to allow controlled slippage between the object and parallel grippers. The work of \cite{Shi2017} controlled the force distribution of a pinch grasp to predict sliding directions. Similarly, \cite{Chen2021} controlled the sliding velocity of an object grasped by a parallel gripper. %Dynamic manipulation may also include releasing the object into mid air and re-grasping in a different orientation \citep{SintovInHand2017}. 

In intrinsic manipulation, the available DOF of the gripper are exploited for manipulating the grasped object \citep{Cruciani2018b}. While jaw grippers have only one DOF, some work has been done to augment their intrinsic manipulation capabilities. Seminal work by \cite{Nagata1994} proposed six gripper mechanisms with an additional one DOF at the tip, each having the ability to either rotate or slide an object in some direction. Similarly, a passively rotating mechanism was integrated into the fingers of the gripper allowing the object to rotate between the fingers by gravity \citep{Terasaki1998}. \cite{Zhao2020} augmented a jaw gripper tip with a two DOF transmission mechanism to re-orient and translate randomly placed screws. \cite{Zuo2021} added a linear actuation along each of the two fingers to enable translation and twist of a grasped object. Similarly, a rolling mechanism was added to the gripper by \cite{Chapman2021} in order to manipulate a flat cable. In-hand manipulation was also enabled for a minimal underactuated gripper by employing an active conveyor surface on one finger \citep{Ma2016}. \cite{Taylor2020} included a pneumatic braking mechanism in a parallel gripper in order to transition between object free-rotation and fixed phases. The above augmentation methods for parallel grippers are limited to one manipulation direction and yield bulky mechanisms that complicate the hardware. However, a simple vibration mechanism was recently proposed to enable $SE(2)$ sliding motion of a thin object between the jaws of a parallel gripper \citep{Nahum2022}.

% \subsubsection{Multi-finger hands}
% Figure \ref{fig:hands}b

\subsubsection{Soft hands}

Soft hands are robotic grippers that are comprised of soft or elastic materials. Due to their soft structure, they usually provide passive compliance upon interaction with the environment \citep{Zhou2018}. Hence, they can grasp objects of varying sizes and shapes without prior knowledge. A class of soft hands is the \textit{pneumatic-based hands} where stretchable fingers can be inflated to generate a grasp. For instance, RBO Hand 2 is a compliant, under-actuated anthropomorphic robotic hand \citep{Deimel2014}. Each finger of the hand is made of cast silicon wrapped with inelastic fabric. When inflated, the fabric directs the stretch of the fingers toward a compliant grasp. %This hand is able to achieve 31 out of 33 identified human grasp postures \citep{feix2015grasp}.
In-hand manipulation with pneumatic-based hands was demonstrated for which heuristic finger gait enabled continuous object rotation (Figure \ref{fig:hands}c) \citep{Abondance2020}. Another pneumatic hand with reconfigurable fingers and an active palm was designed to enable in-hand dexterity while maintaining low mechanical complexity \citep{Pagoli2021}. \cite{Batsuren2019} presented a soft robotic gripper for grasping various objects by mimicking in-hand manipulation. It consists of three fingers, where each of them contains three air chambers: two side chambers for twisting in two different directions and one middle chamber for grasping. The combination of these air chambers makes it possible to grasp an object and rotate it.

An important class commonly referred as a soft hand is the \textit{Underactuated} or \textit{Compliant} hand \citep{Dollar2010,Liu2020}. While the links of such a hand are generally rigid, each finger has compliant joints with springs where a tendon wire runs along its length and is connected to an actuator (Figure \ref{fig:hands}d). Such a structure enables a two or more finger hand to passively adapt to objects of uncertain size and shape through the use of compliance \citep{Odhner2011}. They can, therefore, provide a stable and robust grasp without tactile sensing or prior planning, and with open-loop control. In addition, due to the low number of actuators, they enable a low-cost and compact design. Recently, open-source hardware was distributed for scientific contributions and can be easily modified and fabricated by 3D printing \citep{Ma2017YaleOP}. Along with good grasping capabilities, precise in-grasp manipulation was shown possible \citep{odhner2015stable}. Using visual servoing along with a linear approximation of the hand kinematics, closed-loop control of a two-finger hand was demonstrated \citep{calli2016vision} and later used to track paths planned with an optimization-based model-free planner \citep{calli2018path}. However, a precise analytical model for such hands is not easy to acquire due to the compliance and inherent fabrication uncertainties. Therefore, data-based models were proposed and will be discussed later.

% -------------------------------------------------------------------

\subsection{In-hand manipulation with Dexterous hands}
% Dexterous robotic hand

\cite{Mason1985} claimed that rigid hands can acquire controllability of an object with at least three fingers of three joints each. Such a hand control is termed dexterous manipulation and the hand is a \textit{dexterous hand}. Naturally, grippers that satisfy this dexterity condition are bio-inspired or anthropomorphic \citep{LlopHarillo2019} (Figure \ref{fig:hands}b). Early work on dexterous anthropomorphic hands includes a three-finger and 11-DOF hand \citep{okada1979object}, the four-finger Utah/MIT hand \citep{Jacobsen1986}, and later the Barrett and DLR hands \citep{Townsend2000,Butterfass2001}. Furthermore, extensive work was done on five-finger anthropomorphic hands. Similar to the DLR hand, The Gifu Hand used 16 built-in servo-motors in the joints \citep{Mouri2002}. On the other hand, the Robotnaut hand was designed for space usage and included flex shafts for bending the fingers \citep{Lovchik1999}. A hand from Karlsruhe used 13 flexible fluidic actuators for a lightweight design \citep{Schulz2001}. The UB hand is a five-finger anthropomorphic hand that used elastic hinges to mimic human motion \citep{Lotti2004}.

While recent work on in-hand manipulation with dexterous hands is based on learning approaches, earlier and few recent ones have proposed non-data-driven methods. For instance, the work by \cite{Furukawa2006} proposed a high-speed dynamic regrasping strategy with a multi-fingered hand based on visual feedback of the manipulated object. A different work introduced a planning framework for an anthropomorphic hand to alternate between finger gait and in-grasp manipulations \citep{Sundaralingam2018}. Recent work by \cite{Pfanne2020} used impedance control for stable finger gaiting over various objects with a dexterous multi-finger hand.

% -------------------------------------------------------------------

\subsection{Perception}

Humans use both visual feedback and touch perception for interacting with the environment and, in particular, manipulate objects within their hand \citep{RoblesDeLaTorre2001}. Such sensory modules have been widely explored in robotics, both individually and combined. 

\subsubsection{Vision}

Different variations of visual perception are used to observe a manipulated object and estimate its pose in real time. The easiest application is the positioning of \textit{fiducial markers} such as ArUcO \citep{GarridoJurado2014} or AprilTags \citep{Olson2011}. These markers provide instant pose recognition of a rigid object without the need for geometry recognition \citep{Kalaitzakis2021}. However, the requirement to apply them on an object prevents spontaneous unplanned interaction with an object. In addition, the markers are required to be continuously visible to the camera. Hence, they are commonly for manipulation of specific known objects, or for prototyping. For instance, fiducial markers were used in visual servoing \citep{Calli2017} and hand state representation \citep{Sintov2019} during in-grasp manipulation of an object with an underactuated hand.

Visual pose estimation, which is based on geometry recognition of the object, is usually based on an RGB (monocular) camera, depth camera or both (RGB-D). With RGB data, much work has been done to regress 2D images to spatial pose of objects \citep{Rad2017,Billings2019,Kokic2019}. Nevertheless, in simpler applications where the object is known, it can be segmented using image processing tools. For instance, a high-speed vision system was used by \cite{Furukawa2006} to track a cylinder thrown and caught by a multi-finger hand. Similarly, a high-speed camera was used to solve a Rubik's cube with a fast multi-finger hand \citep{Higo2018}. A work by OpenAI used three RGB cameras to train a model for pose estimation of a cube manipulated by the Shadow hand \citep{andrychowicz2020learning}. \cite{ichnowski2021dex} presented Dex-NeRF, a novel approach that enables grasping using Neural Radiance Field (NeRF) technique. NeRF receives five-dimensional vectors as input and can be used for grasping transparent objects. The RGB values are calculated using an Artificial Neural Network (ANN) only after the initial stages.

Contrary to RGB cameras, 3D sensing such as stereo cameras, laser scanners and depth cameras enable direct access to the distance of objects in the environment. RGB-D sensing, in particular, provides an additional point cloud corresponding to the spatial position of objects in view. For instance, an RGB-D camera was used to estimate the pose of objects before and during grasp by a soft hand \citep{Choi2017}. Similar work involved a depth camera to demonstrate robust pose estimation of objects grasped and partly occluded by a two-finger underactuated hand \citep{Wen2020}. Although visual perception can provide an accurate pose estimation of a manipulated object, it requires a line of sight. Hence, it cannot function in fully occluded scenes and may be sensitive to partial occlusions. Haptic-based approaches can, therefore, provide an alternative or complementary solution. 

\subsubsection{Haptics}

Information from haptic sensors is acquired through direct contact with objects by either tactile sensing or internal sensing of joint actuators known as Kinesthetic (or Proprioception) haptics \citep{Carter2005}. Traditionally, tactile refers to information received from touch sensing, while kinesthetic refers to internal information of the hand sensed through movement, force or position of joints and actuators. While kinesthetic haptics can be easier to measure, tactile sensing is the leading haptic-based sensing tool for object recognition and in-hand manipulation. State-of-the-art tactile sensors include force sensors on fingertips, arrays of pressure sensors \citep{Bimbo2016} or high-resolution optical sensors \citep{yuan2017gelsight,Sun2022,taylor2022gelslim,Azulay2024}. With these sensors, robotic hands can continuously acquire information about the magnitude and direction of contact forces between them and the manipulated object during interaction. An array of pressure sensors was used for servo control of the Shadow hand in in-hand manipulation tasks of deformable objects \citep{Delgado2017}. Another work used optical sensors to learn in-hand manipulation models \citep{lambeta2020digit}. To combine the advantages of haptics and visual perception, some work has been done with both to explore the hand-object interaction during in-grasp manipulation \citep{He2015}.


% ----------------------------------------------------------------------


% \subsection{Older version}
% The survey paper \citep{kawasaki2019humanoid} mentions the applications for Humanoid Robot Hand. Among the relevant applications for this approach, we can mention: breast palpation training system, measurement system for breast engorgement, surgery training system using plural devices, skill transfer system, Finger rehabilitation support system, Virtual robot teaching system, and  electromyogram prosthetic hands. \\
% The first categorization of grasps based upon anthropomorphic perspective \citep{Schlesinger1919} is divided into six types: cylindrical, tip, hook, palmar, spherical and lateral. These grasps are primarily defined by object geometry, but grasp choice is also determined by the task being performed.

% %The point is what the hand holds, how it holds (approach)
% As a baseline of extremely faithful bio-mimicry, consider the  Anantomically Correct Testbad (ACT) hand \citep{deshpande2011}, which mimics both the bone structure and movement transfer mechanism (i.e tendons) of the human hand, as well as the ranges of motion for each joint. The ACT hand is hyper-actuated, with six motors serving as muscles for each finger, except the thumb actuated by eight motors. The wrist is actuated by further four muscles, for a total of 36 actuated DOF. This biologically accurate model is capable of every human hand pose, and is extremely dexterous.
% In comparison, \citep{plappert2018multi} present an environment for learning dexterous manipulation using the Shadow Dexterous Hand model, integrated with OpenGym. 

% A survey of human grasps analysis in literature \citep{feix2009,feix2015grasp} produced a comprehensive set of 33 grasp postures for single-handed orientation-invariant grasps. This set has been used as a measure of robot hand dexterity, aimed especially at under-actuated robots. \citep{Deimel2014} offer a compliant, under-actuated, and dexterous anthropomorphic robotic hand based on soft robotics technology. This hand is able to achieve 31 out of 33 grasp postures mentioned in the human grasp set.

% Acccording to \citep{Lai2020} in order to design humanoid robot hands the designer has to relate to the following characteristics: size, finger DOF, opposability of the thumb, force sensor, built-in servomotor method and unit design of the finger. \citep{nanayakkara2017role} further emphasizes the importance of the role of the thumb in dexterous manipulation tasks, reviewing both the biological human system and its mimicry by existing robotic systems.  

% %Ability to handle soft and hard devices!!!
% %Another perspective is the sensors (vision) simulation of the environment!!!!
% \citep{GamaMelo2014} present an anthropomorphism approach for dexterity that uses indices in order to evaluate and compare between human hand dexterity features. As already mentioned above \citep{GamaMelo2014} divides anthropomorphism into the following categories: kinematics, contact surfaces and size. Each of previous index classes are linearly combined with weights and the result indicates the overall proximity to human hand functionality.
% \citep {GamaMelo2014} defines the the dexterous robotics hand’s challenges as capability of carrying out a powerful hold, as well as having fine manipulative
% skills and versatility. Additional way to categorize the grasp in anthropomorphism approach is the geo metric. Geo metric can be sub divided into power grasp, span grasp, cylindrical grasp, chuck grasp, hook grip, lateral pinch, pulp pinch and precision pinch.

% Additional reason for adapting the anthropomorphism approach mentioned by \citep {GamaMelo2014} relies on the fact that there is a need for human multi finger in order to manipulate human-centered objects. This manipulation requires precise motion and force control that cannot be achieved by generic robotic gripper. The need for multipurpose device that function on variety of daily needs is also an accelerator for mimicking human hand’s main features. 
% In addition to sensory robotic system there is a need for mechanical design that will connect in efficient way between actuators, sensors and transmission mechanism \citep {GamaMelo2014}.

% \citep{GamaMelo2014} offers an evaluation method based upon the following features: size, weight, flexibility, precision, hysteresis, energy consumption, potency, efficiency, and components cost.
% \citep {Xu2016,xu2018approaching} believes that the biomechanics of human hand is an essential component of the hand dexterity and can be replicated with highly bio-mimetic design. They also offer a different hand taxonomy realized by our bio-mimetic robotic hand. They divide between power grasp and precision grasp. The last class is divided into circular and prismatic. The power grasp category can be divided into prehensile, non prehensile, circular and prismatic.

% In order to achieve better performance while using anthropomorphism approach \citep{GamaMelo2014} offers to distinguish between different tactile sensor types. The different types are human oriented levels of senses. \citep{GamaMelo2014} differs between modalities of the sensor: normal pressure, skin deformation and dynamic tactile sensing. 
% In addition, in order to assess the input motion and force sources, different types of actuators are used. The actuators are classified by their operating principle of motion generation. \citep{GamaMelo2014} mentions the conventional and non-conventional classes. The conventional class is sub divided into electric, hydraulic and pneumatic.

% Another perspective that links between robots dexterity to human hand using the anthropomorphism approach is the control system. \citep{GamaMelo2014} define control variables such as joints angle position on the fingers, velocity of the links, or force on the grasping. In addition, the robotic hand control system has to take into account position control and force control. Position control guarantees a minimum error in the following steps to the desired movement. The outcome of the position control is obtained by the joints position of the grasping process. Each position depends on the grasped object shape. \citep{GamaMelo2014} mention two classic strategies: PID (also known as Hard Control techniques) and calculated torque. 

% \citep{Lai2020} introduce control haptic interface. The unique characteristics of the control system and its interface determine the functionality of robot hand and its applications. The interface can be activvated manually or by voice, EMG, EEG, telemanipulation or by eye pupils positions. 

% Additional way to mimic human-being using anthropomorphism approach is using biological hand movement while covering discontinuous surface \citep{GamaMelo2014}. Another strategy is based on sEMG and EMG. It is a control strategy that is based on signals taken in hand and arm muscles \citep{dwivedi2019learning,kwon2021electromyography}. Usually it is implemented when there is no way to assess the force feedback from the hand or fingers. The this control techniques indicates the grasping positions basing in the muscles as well as the signals and provides a feedback to the controller.

% There are many techniques and approaches for improving robot dexterity by using anthropomorphism approach. \citep {Kontoudis2019, Kontoudis2018} present an adaptive robot hand that is capable of performing selective interdigitation, robust grasping,and dexterous, in-hand manipulation. The novelty in their design relies on under-actuated, compliant, anthropomorphic robot fingers that are implemented with flexure joints based on elastomer materials. The design also consists of metacarpophalangeal (MCP) joint of each finger can achieve both flexion/extension and abduction/adduction.

% V \citep{Batsuren2019} present a soft robotic gripper for grasping various objects by mimicking in-hand manipulation. It consists of three fingers, where each of them contains three air chambers: two chambers (side chambers) for twisting in two different directions and one chamber (middle chamber) for grasping. The combination of these air chambers makes it possible to grasp an object and rotate it.

% \citep{Kumar2016a} introduce dynamic dexterous manipulation on physical hardware. This Adroit hand comes into practice by 28 degrees of freedom arm-hand system capable of hosting dexterous dynamics manipulation, based on pneumatic actuation system. In addition, a behavior synthesis technique is mentioned. This technique mimics human hand in a way that it synthesizes the details of dynamic dexterous manipulation in high dimensional manipulators in scalable way. 

% \citep{Ludersdorfer2016} introduce TacHand, a tactile robotic hand with in-hand manipulation capabilities. The results of the work show the importance of the abstraction of the functionality of  human hand for the development of dexterous robotic hands, and the necessity to convert these abstractions into simple mechanical solutions as well as to mathematical model.

% \citep{Xu2013, Xu2013a} describe method of designing and modelling of a 20-DOF anthropomorphic robotic hand. Their robotic hand a has 31 components, and can be manufactured while changing parameters such as finger length, DOF, and ROM (range of motion). In addition they use Skin pads for tactile sensing. Their unique robot hand is based upon developing optimal control techniques and can be manufactured in less than 24 hours.

% For summing this Humanoid robot hands section we can cite \citep {Xu2016} who believe that the biomechanics of human hand is an essential component of the hand dexterity and can be replicated with highly bio-mimetic design. At this time, our are evident to research that reinterpret the important bio-mechanical advantages of the human  hand  from  robotic  perspective. Our survey show that the design of a bio-mimetic robotic hand mimics human counterpart with artificial joint capsules,crocheted ligaments  and  tendons, laser-cut extensor hood and  elastic-pulley mechanisms. \citep {Xu2016} experimentally identify the workspaces of the fingertips and successfully demonstrate that our proof-of-concept design can be teleoperated to grasp and manipulate daily objects with a variety of natural hand postures based on hand taxonomy.

==> sum_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\centering
\caption{Summary of state-of-the-art work on learning approaches for in-hand manipulation (in alphabetical order)}
\label{tb:Pcomparison}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l ccc c c c ccc}\toprule
\multirow{2}{*}{Paper} & \multicolumn{3}{c}{Learning type} & Manipulation & Dex./Non-Dex. & Rigid/Soft       & \multicolumn{3}{c}{Perception} \\\cline{2-4}\cline{8-10}
 & Model        & RL       & IL       &   type   & hand  & hand & Vision   & Tactile   & Kines.  \\\midrule

\rowcolor{Gray}
\cite{allshire2022transferring} & & \checkmark &  & In-Grasp & Dex. % edge of dexterity, three dexterous fingers
& Rigid & \checkmark & & \checkmark \\

\cite{antonova2017reinforcement} & & \checkmark & & Pivoting & Non-Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{OpenAI2019,andrychowicz2020learning} & & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Arunachalam2023,Arunachalam2023holo} & & & \checkmark & Mix & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{azulay2022learning} & \checkmark & & & In-grasp & Non-Dex. & Soft & & \checkmark  & \checkmark\\

\cite{azulay2022haptic} & & \checkmark & & In-Grasp & Non-Dex. & Soft & & & \checkmark\\

\rowcolor{Gray}
\cite{Calli2018} & \checkmark & & & In-Grasp & Non-Dex & Soft & \checkmark & & \checkmark \\

\cite{chen2021simple,chen2022} & & \checkmark & & Mix & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Chen2023} & & \checkmark & & F. Gait & Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Cruciani2017,Cruciani2018} & & \checkmark & & Pivoting & Non-Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{deng2020learning} & & & \checkmark & Mix & Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Dimou2023} & \checkmark & & & In-Grasp & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Falco2018} & & \checkmark & & In-Grasp & Dex. & Soft & \checkmark & \checkmark &  \\

\cite{funabashi2019morphology,funabashi2020variable,Funabashi2019} & & \checkmark & & Rolling & Dex. & Rigid %with soft fingertips
& & \checkmark & \checkmark % is the kines. not always true?
\\

\rowcolor{Gray}
\cite{GarciaHernando2020} & & & \checkmark & Mix & Dex & Rigid & \checkmark & & \\

\cite{Gupta2021} & & \checkmark & &  Mix & Dex. & Rigid & \checkmark &  &  \\ 

\rowcolor{Gray}
\cite{Handa2023} & & \checkmark & & Mix & Dex. & Rigid & \checkmark & & \\ 

\cite{Huang2021} & & \checkmark & & F. Gait & Dex. & Rigid & \checkmark &  & \\

\rowcolor{Gray}
\cite{Jain2019} & & \checkmark & \checkmark & In-Grasp & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\cite{Khandate2022,Khandate2023} & & \checkmark & & F. Gait & Dex. & Rigid & & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{kimmel2019belief} & \checkmark & & & In-Grasp & Non-Dex. & Soft & \checkmark & & \checkmark \\

\cite{korthals2019multisensory} & & \checkmark & & Mix & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{Kumar2016b} & & & \checkmark & Mix & Dex. & Rigid & & \checkmark & \checkmark \\

\cite{Li2014} & & & \checkmark & In-grasp & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{Li2020} & \checkmark & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark 
\\ % In general I used In-grasp to describe manipulations where it seems the object is grasped during the entire motion, and combination when it is "released" to move dynamically at least for part of the motion.

\cite{luo2023} & \checkmark & & & Mix & Dex. & Rigid & \checkmark & & \checkmark \\

\rowcolor{Gray}
\cite{melnik2021} & & \checkmark & & Mix & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\cite{morgan2020object} & \checkmark & & & In-Grasp & Non-Dex. & Soft & \checkmark & &  \\

\rowcolor{Gray}
\cite{Morgan2021} & \checkmark & \checkmark & & Mix & Non-Dex. & Soft & \checkmark & &  \\

\cite{nagabandi2020deep} & \checkmark & \checkmark & & Mix & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Orbik2021} & & & \checkmark & Mix & Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Park2024} & \checkmark & & & In-Grasp & Non-Dex. & Soft & & \checkmark & \\

\rowcolor{Gray}
\cite{Pitz2023} & & \checkmark & & In-Grasp & Dex. & Rigid & & & \checkmark \\

\cite{qi2022} & & \checkmark & & F. Gait & Dex. & Rigid & & & \checkmark \\

\rowcolor{Gray}
\cite{Qi2023} & & \checkmark & & F. Gait & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\cite{radosavovic2020state} & & & \checkmark & Mix & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Rajeswaran2017} & & & \checkmark & Mix & Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Shin2024} & & & \checkmark & Rolling & Dex. & Rigid & \checkmark & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{Sievers2022} & & \checkmark & & In-Grasp & Dex. & Rigid & & & \checkmark \\

\cite{Sintov2019,sintov2020motion} & \checkmark & & & In-Grasp & Non-Dex. & Soft & \checkmark & & \checkmark \\

\rowcolor{Gray}
\cite{Solak2019} & & & \checkmark & In-Grasp & Dex. & Rigid & & & \checkmark \\

\cite{Solak2023} & & & \checkmark & In-Grasp & Dex. & Rigid & & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{srinivasan2020learning} & & \checkmark & & In-Grasp & Dex. & Rigid & \checkmark & & \checkmark \\ %use same environ., robot, and task and nagabandi2019, need to update sensory after adding that paper

\cite{Tao2023} & & \checkmark & & Mix & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Toskov2023} & \checkmark & & & Pivoting & Non-Dex. & Rigid & & \checkmark & \\

\cite{Toledo2021} & & \checkmark & & Pivoting & Non-Dex. & Rigid & \checkmark & &  \\

\rowcolor{Gray}
\cite{VanHoof2015} & & \checkmark & & In-Grasp & Non-Dex. & Soft & & \checkmark & \\

\cite{Veiga2020} & & \checkmark & & In-Grasp & Dex. & Rigid & & \checkmark & \\

\rowcolor{Gray}
\cite{wang2020swingbot} & \checkmark & & & Pivoting & Non-Dex. & Rigid &  &  & \checkmark \\

\cite{Wei2023} & & & \checkmark & Sliding & Dex. & Rigid & \checkmark & & \\

\rowcolor{Gray}
\cite{Yang2023} & & \checkmark & & Mix & Dex. & Rigid & & \checkmark & \\

\cite{Yin2023} & & \checkmark & & Mix & Dex. & Rigid & & \checkmark & \checkmark \\

\rowcolor{Gray}
\cite{Yuan2020} & & & \checkmark & Rolling & Non-Dex. & Rigid & \checkmark & & \checkmark \\

\cite{Yuan2023} & & \checkmark & & Mix & Dex & Rigid & \checkmark & \checkmark & \checkmark \\

\bottomrule                  

\end{tabular}
\end{adjustbox}

\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
